A Stochastic Proximal Polyak Step Size

Recently, the stochastic Polyak step size (SPS) has emerged as a competitive adaptive step size scheme for stochastic gradient descent. Here we develop ProxSPS, a proximal variant of SPS that can handle regularization terms. Developing a proximal variant of SPS is particularly important, since SPS requires a lower bound of the objective function to work well. When the objective function is the sum of a loss and a regularizer, available estimates of a lower bound of the sum can be loose. In contrast, ProxSPS only requires a lower bound for the loss which is often readily available. As a consequence, we show that ProxSPS is easier to tune and more stable in the presence of regularization. Furthermore for image classification tasks, ProxSPS performs as well as AdamW with little to no tuning, and results in a network with smaller weight parameters. We also provide an extensive convergence analysis for ProxSPS that includes the non-smooth, smooth, weakly convex and strongly convex setting.

==> aux_lemma.tex <==
\fabian{All below: not used, but might be useful}
\begin{lemma}
\label{lem:bound-squared-grad}
Let $f:\R^n \to \R$ be bounded from below and $L$--smooth. Then, for all $x\in \R^n$ it holds
\begin{align}
    \label{eqn:bound-grad}
    \frac{1}{2L}\|\nabla f(x)\|^2 \leq f(x)- \inf f.
\end{align}
\end{lemma}
%
\begin{proof}
From Lipschitz-smoothness, we obtain that for all $x,y \in \R^n$ it holds
\begin{align*}
   \inf f\leq f(y) \leq f(x) + \iprod{\nabla f(x)}{y-x} + \frac{L}{2}\|y-x\|^2.
\end{align*}
Minimizing the right-hand side over $y$, the minimum is attained at $\hat y = x- \oneover{L}\nabla f(x)$. Plugging in yields
\begin{align*}
   \inf f\leq f(x) - \iprod{\nabla f(x)}{\oneover{L}\nabla f(x)} + \frac{L}{2}\|\oneover{L}\nabla f(x)\|^2 = f(x) - \oneover{2L}\|\nabla f(x)\|^2.
\end{align*}
\end{proof}
%
\begin{lemma}
\label{lem:bound-squared-grad-reg}
Let $f:\R^n \to \R$ be bounded from below and $L$--smooth. Then, for all $x\in \R^n$ and all $\beta>0$ it holds
\begin{align}
    \label{eqn:bound-grad-reg}
    \frac{1}{2}\|\nabla f(x)\|^2 - \frac{\beta L}{2}\|x\|^2 \leq (L+\beta)(f(x)- \inf f) - \beta \iprod{\nabla f(x)}{x}.
\end{align}

\end{lemma}
%
\begin{proof}
Let $\beta >0$. From Lipschitz-smoothness we obtain that for all $x,y \in \R^n$ it holds
\begin{align*}
   \inf f \leq f(y) + \frac{\beta}{2} \|y\|^2 \leq f(x) + \iprod{\nabla f(x)}{y-x} + \frac{L}{2}\|y-x\|^2 + \frac{\beta}{2} \|y\|^2.
\end{align*}
The right-hand-side is minimized (over $y$) by $\hat y = \frac{1}{1+\beta/L}(x-\frac{1}{L}\nabla f(x)) = \prox{\frac{\beta}{2L}\|\cdot\|^2}(x-\frac{1}{L}\nabla f(x))$. Plugging in $\hat y$ for $y$ yields
\begin{align*}
    \inf f &\leq  f(x) + \iprod{\nabla f(x)}{-\tfrac{\beta}{L+\beta}x-\tfrac{1}{L+\beta}\nabla f(x)} + \frac{L}{2}\|-\tfrac{\beta}{L+\beta}x-\tfrac{1}{L+\beta}\nabla f(x)\|^2 \\
    & \quad + \frac{\beta}{2}\|\tfrac{1}{1+\beta/L}(x-\tfrac{1}{L}\nabla f(x))\|^2 \\
    &= f(x) + \|x\|^2\big[\tfrac{L\beta^2}{2(L+\beta)^2} + \tfrac{L^2\beta}{2(L+\beta)^2}\big] 
    + \iprod{\nabla f(x)}{x}\big[-\tfrac{\beta}{L+\beta} +L\tfrac{\beta}{(L+\beta)^2}- \beta\tfrac{L}{(L+\beta)^2} \big] \\
    &\quad + \|\nabla f(x)\|^2\big[-\tfrac{1}{L+\beta} + \tfrac{L}{2(L+\beta)^2} + \tfrac{\beta}{2(L+\beta)^2} \big] \\
    &= f(x) + \tfrac{\beta L}{2(L+\beta)} \|x\|^2 - \tfrac{\beta}{L+\beta}\iprod{\nabla f(x)}{x} - \tfrac{1}{2(L+\beta)}\|\nabla f(x)\|^2
\end{align*}
Multiplying with $L+\beta$ and rearranging yields the result.
\end{proof}
%
%
Recall from \cref{lem:sps-update-unreg} the quantity $\gamma_k = \min \left\{\alpha_k, \frac{f(x^k;S_k)-C_k}{\|g_k\|^2} \right\}$ which can be bounded from below in the Lipschitz-smooth case (cf.\ \cite{Loizou2021}):
\begin{lemma}
\label{lem:gammak-lower-bound}
Assume that $f(\cdot;s)$ is bounded from below and $L_s$--smooth for all $s\in \mathcal{S}$ and let $L_{\max}\geq L_s$ for all $s\in \mathcal{S}$. Then for $\gamma_k$ defined as in \cref{lem:sps-update-unreg} it holds 
\begin{align}
    \label{eqn:lower-bound-gamma}
    \gamma_k \geq \min\left\{\alpha_k, \frac{1}{2L_{\max}}\right\}.
\end{align}
\end{lemma}
\begin{proof}
Note that $f(x^k;S_k) - C(S_k) \geq f(x^k;S_k) - \inf_x f(x;S_k)$. Applying \cref{lem:bound-squared-grad} to $f(\cdot;S_k)$, we have $\frac{f(x^k;S_k)-C(S_k)}{\|\nabla f(x^k;S_k)\|^2} \geq  \frac{1}{2L_{\max}}$
and thus 
\[\gamma_k = \min \left\{\alpha_k, \frac{f(x^k;S_k)-C(S_k)}{\|g_k\|^2} \right\} \geq \min\left\{\alpha_k, \frac{1}{2L_{\max}}\right\}.\]
\end{proof}
%
%
\begin{lemma} \label{lem:phi-ineq}
Let $h: \R^n\to \R$ be closed convex. Let $x,d\in\R^n$ and $\alpha,\tau > 0$. If
\[y=\prox{\alpha h}(x-\tau d),\]
then for all $z\in\R^n$ it holds
\[h(y) + \frac{\tau}{\alpha}\iprod{y-z}{d} \leq h(z) + \frac{1}{2\alpha}\big[\|z-x\|^2 - \|y-z\|^2 -\|y-x\|^2 \big]. \]
\end{lemma}
\begin{proof}
Use \cite[Lem.\ 5]{J.Reddi2016} with $h=h,~\eta=\alpha,~x=x-\tau d$ and rearrange.
\end{proof}
%
\begin{lemma}
\label{lem:bound-with-noise}
Assume that $f$ is bounded from below and $f(x)=\E[f(x;S)]$. Assume that, for all $s\in \mathcal{S}$, the function $f(\cdot;s)$ is bounded from below and $L_s$--smooth. Moreover, let $L_{\max} \geq L_s$ for all $s\in \mathcal{S}$.
Defining
\[\sigma^2 := \inf f - \E[\inf_x f(x;S)] \geq 0,\]
for all $x\in\R^n$ it holds
\begin{align*}
    \E\|\nabla f(x;S)\|^2 \leq 2L_{\max}(f(x)-\inf f+ \sigma^2). 
\end{align*}
\end{lemma}
%
\begin{proof}
Applying \cref{lem:bound-squared-grad}, for all $s\in \mathcal{S}$ and $x\in \R^n$ it holds
\begin{align*}
    \frac{1}{2L_{\max}}\|\nabla f(x;s)\|^2 \leq \frac{1}{2L_s}\|\nabla f(x;s)\|^2 \leq f(x;s)- \inf_x f(x;s).
\end{align*}
Now, applying expectation and adding $0=\inf f - \inf f$ to the right-hand side gives the claimed result.
\end{proof}
%
\begin{lemma}
Let $a,b,c \in \R$. Then, $\max\{a,c\} -\max\{b,c\} \leq \max\{a-b,0\}$.
\end{lemma}
\begin{proof}
We do a case distinction and denote $L:= \max\{a,c\} -\max\{b,c\}$ and $R:=\max\{a-b,0\}$.
\begin{enumerate}
    \item $a>c$ and $b>c$. Then $L=a-b$ and $R\geq a-b$.
    \item $a<c$ and $b<c$. Then $L=0$ and $R\geq 0$.
    \item $a>c$ and $b<c$. Then $L=a-c$ and $R \geq a-b \geq a-c $.
    \item $a<c$ and $b>c$. Then $L= c-b \leq 0$ and $R\geq 0$.
\end{enumerate}
\end{proof}
%
